Symbolic Parallel Composition for Multi-language Protocol Verification

The implementation of security protocols often combines different languages. This practice, however, poses a challenge to traditional verification techniques, which typically assume a single-language environment and, therefore, are insufficient to handle challenges presented by the interplay of different languages. To address this issue, we establish principles for combining multiple programming languages operating on different atomic types using a symbolic execution semantics. This facilitates the (parallel) composition of labeled transition systems, improving the analysis of complex systems by streamlining communication between diverse programming languages. By treating the Dolev-Yao (DY) model as a symbolic abstraction, our approach eliminates the need for translation between different base types, such as bitstrings and DY terms. Our technique provides a foundation for securing interactions in multi-language environments, enhancing program verification and system analysis in complex, interconnected systems.

==> macros-tikz-styles.tex <==
\usepackage{tikz}
\usepackage{tikz-cd,tkz-base,tkz-fct}

\usetikzlibrary{decorations.pathreplacing,angles,quotes}
\usetikzlibrary{shapes.geometric, arrows}
\usetikzlibrary{positioning,arrows.meta}

\definecolor{lightblue}{rgb}{0.68, 0.85, 0.9}
\tikzset{
	block/.style={
		draw, 
		rounded corners,
		text width=15em,
		text centered,
		minimum height=5ex,
		fill=lightblue
	},
	line/.style={
		draw, 
		-Stealth
	},
}
\tikzset{
	block1/.style={
		draw, 
		rounded corners,
		text width=20em,
		text centered,
		minimum height=5ex,
		fill=cyan!30!white
	},
	line/.style={
		draw, 
		-Stealth
	},
}
\tikzstyle{process} = [rectangle, minimum width=2cm, minimum height=1cm, text centered, text width=2cm, draw=black, fill=orange!30]
\tikzstyle{process1} = [rectangle, minimum width=1cm, minimum height=1cm, text centered, text width=1cm, draw=black, fill=orange!30]
\tikzstyle{arrow} = [thick,->,>=stealth]


==> sections/BIR-Exp4.tex <==

\let\origthelstnumber\thelstnumber
\makeatletter

\renewcommand\thelstnumber{%
    \ifnum\value{lstnumber}<7
        \origthelstnumber
    \else
        \ifnum\value{lstnumber}>7
            $|$
        \fi
    \fi
}

\tcbset{
  myfancybox/.style={
  titlerule=1pt, 
  boxsep=0pt, 
  colframe=mGray, 
  halign=left, 
  valign=center,
  left=0pt, right=0pt, top=0pt, bottom=0pt, 
  title={\hspace{1.5em}$\birsymb$ Statement\hspace{5em}$\sbirsymb$ Predicate\hspace{1em}$\sbirsymb$ Event\hspace{3.2em}$\SapicOld$ Process\hspace{3.5em}DY Predicate\hspace{1.8em}Via $ \dedrelcombSbirDY $}
    }
}
\begin{figure*}
\begin{tcolorbox}[myfancybox]
    \noindent%
    \begin{minipage}{0.25\textwidth}
\begin{lstlisting}[style=asmstyle]
[R30$\fstlangcol{=}\textcolor{mGreen}{1}$;]$\fstlangcol{jmp}$(0x44)//$\mathlabel{rng}$
$\fstlangcol{assign}$(R1, $\fstlangcol{var}$(R0))
$\fstlangcol{assign}$(R0, $\fstlangcol{m}$)
[R30$\fstlangcol{=}\textcolor{mGreen}{4}$;]$\fstlangcol{jmp}$(0x20)//$\mathlabel{senc}$
[R30$\fstlangcol{=}\textcolor{mGreen}{5}$;]$\fstlangcol{jmp}$(0x04)//$\mathlabel{send}$
$\fstlangcol{assign}$(R2, R1$\fstlangcol{\oplus 0xde..}$)
[R30$\fstlangcol{=}\textcolor{mGreen}{7}$;]$\fstlangcol{jmp}$(0x04)//$\mathlabel{send}$
\end{lstlisting}
    \end{minipage}%
    \begin{minipage}{0.145\textwidth}
 \begin{lstlisting}[style=birstyle, firstnumber = 8]
-
$ \progEqual{R1}{\fstlangcol{var}(k)} $
$ \progEqual{R0}{\fstlangcol{m}} $
$ \progAliEq{c}{\mathlabel{senc}(R0,R1)} $
-
$ \progEqual{R2}{R1\fstlangcol {\oplus 0xde..}} $
-
\end{lstlisting}
    \end{minipage}%
    \begin{minipage}{0.17\textwidth}
		\begin{lstlisting}[style=birstyle, firstnumber = 8]
$ \Syncfresh{k} $
$ \assign{R1}{\fstlangcol{var}(k)} $
$ \assign{R0}{\fstlangcol{m}} $
$ \fcall{\mathlabel{senc},R0,R1,c} $
$ \PtoA{c} $
$ \assign{R2}{R1\fstlangcol {\oplus 0xde..}} $
$ \PtoA{R2} $
\end{lstlisting}
    \end{minipage}%
 \begin{minipage}{0.20\textwidth}
	\begin{lstlisting}[style=birstyle, firstnumber = 8]	
$ \pnew~k; $
$ \plet~R1 = k~\pin $
$ \plet~R0 = m~\pin $
$ \plet~c = \mathlabel{senc}(R0,R1)~\pin $
$ \pout(c); $
$ \plet~R2 = \functionsymbol{xor}(R1,\constrans{de..})~\pin $
$ \pout(R2); $
\end{lstlisting}
\end{minipage}%
    \begin{minipage}{0.145\textwidth}
		\begin{lstlisting}[style=birstyle, firstnumber = 8]
$\freshness{k}$
-
-
$\dyAliEq{c}{\mathlabel{senc}(R0,R1)} $
$ \knowledge{c} $
-
$ \knowledge{R2} $
\end{lstlisting}
    \end{minipage}%
    \begin{minipage}{0.9\textwidth}
		\begin{lstlisting}[style=birstyle, firstnumber = 8]
-
$ \knowledge{k} \hspace{1.5em} (2)$
-
-
$ \knowledge{R0} \hspace{0.8em} (3)$
-
$ \knowledge{R1} \hspace{0.8em} (1)$
\end{lstlisting}
    \end{minipage}
\end{tcolorbox}
\caption{The sequence of $\birsymb $ statements of~\Cref{ex:masked-encryption}, along with the corresponding updates resulting from symbolic execution, model extraction and the deduction combiner $ \dedrelcombSbirDY $. $\constrans{de..}$ represents the constant value $ \fstlangcol{0xde..}$. \newrevised{Jumps (at lines 0, 3, 4, and 6) are the translation of \textit{branch and link} instruction used for function calls in ARM, which requires updating the \textit{link register} $ R30 $. We present this register update in $[..]$ to mean that it is not relevant to what we intend to present in this example. }}
\label{fig:bir-exp4}
\end{figure*}

==> sections/SBIR.tex <==
\section{Case study: symbolic BIR}
\label{sec:sbir}

We build our work on an existing proof-producing symbolic execution for BIR~\cite{proofproducingsymbexecution}.
It formalizes the symbolic generalization of BIR (hereafter SBIR), i.e., a single-step semantics with an environment containing symbolic
expressions and path conditions constraining those expressions.
%
The symbolic semantics is bisimilar to the concrete semantics and
provides a means to guide the symbolic execution while maintaining a sound set of reachable symbolic states from an initial symbolic state (we call this the symbolic execution structure).

To symbolically generalize from BIR to SBIR, symbolic expressions $\sbirvals$ are defined. Such expressions can be interpreted to BIR values $\birval$ or symbols $ \symbset $ via an interpretation $\sbirvaluation : \sbirvals \to \birval \uplus \symbset$ that assigns BIR values or symbols to an expression's symbols to finally evaluate the whole expression to a BIR value or a symbol.
%
In addition to the environment and program counter,
and SBIR state
$\tuple{\sbirpcond, \sbirenv, \birpc} \in \sbirstates{}$
also contains
a path condition $\sbirpcond$, which is a symbolic expression ($\sbirpcond \in \sbirvals$).
%
Also, the environment maps BIR variables to symbolic values (i.e., symbolic expressions) $\sbirenv: \birvar \mapsto \sbirvals$. 
%
By contrast,
the program counter is kept concrete,
meaning the symbolic execution considers concrete control flow, as opposed to symbolic program counter values.

Having extended the notion of symbolic value interpretation to symbolic environment interpretation, one obtains the notion of matching a symbolic state with a concrete state.
This requires, first, their program counters to be equal.
Second,
given
a symbol interpretation $H$, 
the interpreted symbolic environment equals the concrete environment.
Third, interpreting the path condition $\sbirpcond$ results in the BIR value $\true$.


We use the symbolic execution of a BIR program to get its execution tree which will later be used to obtain the program's SAPIC model. 
%
Each node in the tree is either a branching node 
$\branchingnode(\nodecond, \tree_{\fstlangcol{1}}, \tree_{\fstlangcol{2}})$ with $\nodecond$ a conditional BIR expression and $\tree_{\fstlangcol{i}}$ a sub-tree, or an event node $\node(\birpc, \nodeevent)$.
In event nodes, $\birpc$ is a label which uniquely identifies the program point $\birpc$ where the event occurred.
Leaf nodes are those for which  $\var{ev}$ is set to $\bot$. An edges
connects two nodes iff the transition relation connects
the corresponding symbolic states.

The tree is constructed from a BIR program $\birprog$ and an initial
symbolic state as follows: the root is the initial state. For any
node, including the root, the crypto-aware symbolic execution gives
us up to two successors states.
%
If the node represented a branching statement, we obtain two successor states. We store the statement's condition in a branching node and proceed to translate the two successor states into subtrees.
%
If the node represented any other statement, there can only be one or
no successor state, and we store an event node with, or respectively without,
a successor tree. 
We use the "[]" selection operator to extract the tree node for a give program counter, i.e. $\tree[\birpc]$ will return a node in the tree which is indexed by $\birpc$.

==> sections/trans-to-sapic.tex <==
\section{Model Extraction: Symbolic Exec. to SAPIC}
\label{sec:trans-to-sapic}
\input{gfx/trans-tree-sapic}

\subsection{The \Sapic Language}\label{ssec:sapic}
\input{gfx/syntax-SAPIC}
\input{gfx/sapic-semantics-short}

\Sapic is an applied $\pi$ calculus similar to \ProVerif~\cite{blanchet2001efficient} and \SapicOld~\cite{kremer2016automated}.
\Sapic  is added features to \SapicOld include the definition of destructors, let bindings with pattern matching and else branches.
We present the syntax of \Sapic in~\autoref{fig:SAPICsyntax} where 
$t,st, t_i \in \Term$ range over arbitrary terms, 
$n \in \privnames$ ranges over private names, 
$x \in \Vars$ ranges over variables,  
$p \in \Patterns $ ranges over patterns, and
$ F \in \Facts$ ranges over facts.

\textit{Elementary processes} model finite protocols that
where $\pnew$ construct create fresh values, and 
input and output constructs receive and send messages over a channel $t_1$. 
\textit{Extended processes} model unbounded protocols which may also raise events for model reachability properties. 
\textit{Stateful processes} can manipulate globally shared states $\mathit{st}$, i.e., 
some database, register or memory location that can be read and altered by different parallel threads.

Conditionals are described by first-order formulae $\phi$ over equalities on terms, possibly containing variable quantifiers, as in~\cite{kremer2016automated}.
The \Sapic transition relation is defined based on semantic configurations $ (\Processes,\Subst) \in \sapicconfig $ where 
$ \Processes $ is a set of executable processes, and 
$ \Subst $ is a substitution where its domain contains attacker variables from $\attvars = \{ \att_i \}_{i \in \Nat}$.

$\trans{\ell}{\sapicidx}{}{} \subseteq \sapicconfig \times \Facts \times \sapicconfig$ denotes a labeled transition system that transforms \Sapic semantic configurations where $\ell$ may be empty, or a set of \emph{facts}. 
A multi-step labeled transitions is represented by $P \Trans{l_1\cdot \dots \cdot l_n} \sapicconfig$ where $(\{P\},\emptyset) \trans{}^*\trans{l_1}\trans{}^* \dots\allowbreak
\trans{}^*\allowbreak\trans{l_n}\allowbreak\trans{}^* \sapicconfig$.
Such a sequence of labels defines a \Sapic trace $ \sapicTrace \in \sapictraces $ such that $ \sapicTrace = l_1 \dots l_n $.
We have borrowed  the semantics of the \Sapic transition relations from~\cite{cheval2022sapic+}. 
A few representative transition rules of \Sapic are presented in~\autoref{fig:sapictranssemantics} (see~\autoref{fig:sapictranssemantics-long} in \autoref{app:sapicsemantics} for the full version).

\subsection{To SAPIC}
We now proceed to explain how to automatically extract the SAPIC model from the $\birsymb$ representation of the protocol we analyze. The extracted model should preserve behaviors of the BIR representation and thus ensure that we can transfer back the verified properties at the SAPIC level to BIR and eventually to the binary of the protocol.
Our model extraction approach relies on translating the symbolic execution tree $\tree$ of the protocol under adversarial semantics into its corresponding SAPIC model.
We translate $\tree$ into an executing process $\imlprocessq^{\mathit{full}}$
according to the rules depicted in Fig.~\ref{fig:sbirtosapic}, where $\sbirtoiml{\tree}$ represents the compiled process, i.e. $\imlprocessq^{\mathit{full}} = \sbirtoiml{\tree}$.

Our translation converts $\tree$'s leaf nodes into a \textbf{nil} process $0$. For internal nodes, however, we translate the event stored in each node---extracted by the $\filter{\mathit{events}}$ function---into its SAPIC counterpart. Notice that we do not translate $\tau$ events. Fig.~\ref{fig:sbirtosapic} also presents our rules to translate symbolic $\birsymb$ expressions in the $\tree$'s branching nodes into their corresponding SAPIC terms.
